Few-shot Novel View Synthesis using Depth Aware 3D Gaussian Splatting

3D Gaussian splatting has surpassed neural radiance field methods in novel view synthesis by achieving lower computational costs and real-time high-quality rendering. Although it produces a high-quality rendering with a lot of input views, its performance drops significantly when only a few views are available. In this work, we address this by proposing a depth-aware Gaussian splatting method for few-shot novel view synthesis. We use monocular depth prediction as a prior, along with a scale-invariant depth loss, to constrain the 3D shape under just a few input views. We also model color using lower-order spherical harmonics to avoid overfitting. Further, we observe that removing splats with lower opacity periodically, as performed in the original work, leads to a very sparse point cloud and, hence, a lower-quality rendering. To mitigate this, we retain all the splats, leading to a better reconstruction in a few view settings. Experimental results show that our method outperforms the traditional 3D Gaussian splatting methods by achieving improvements of 10.5% in peak signal-to-noise ratio, 6% in structural similarity index, and 14.1% in perceptual similarity, thereby validating the effectiveness of our approach. The code will be made available at: https://github.com/raja-kumar/depth-aware-3DGS

==> tables/ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\footnotesize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}|l|ccc|@{}}
\toprule
\multicolumn{1}{|c|}{}       & \multicolumn{3}{c|}{\textbf{Average}} \\ \cmidrule(l){2-4} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{Method}}} &
  \multicolumn{1}{c|}{\textbf{SSIM} $\uparrow$} &
  \multicolumn{1}{c|}{\textbf{PSNR} $\uparrow$} &
  \textbf{LPIPS} $\downarrow$ \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}3DGS & 0.694       & 19.57      & 0.319      \\
+ SI Depth                   & 0.698       & 19.77      & 0.312      \\
+ SH=1 &
  \cellcolor[HTML]{FFF2CC}0.703 &
  \cellcolor[HTML]{FFF2CC}20.06 &
  \cellcolor[HTML]{FFF2CC}0.311 \\
+ op\_reset=None &
  \cellcolor[HTML]{FCE5CD}\textbf{0.736} &
  \cellcolor[HTML]{FCE5CD}\textbf{21.64} &
  \cellcolor[HTML]{FCE5CD}\textbf{0.274} \\ \bottomrule
\end{tabular}%
}
\caption{Quantitative ablation study to support the design choices for our experiments. Notice that cascading each method choice results in a gradual increase in the performance, getting the best results with our final proposed method: Scale-Invariant (SI) depth loss, Order of Spherical Harmonics (SH) = 1, and no Opacity (op) reset throughout the training process. The \colorbox[HTML]{FCE5CD}{\textbf{best}} performance numbers are bolded, followed by \colorbox[HTML]{FFF2CC}{second best}.}
\label{table:ablation}
\end{table}
